Causal survival analysis under competing risks using longitudinal modified treatment policies

Longitudinal modified treatment policies (LMTP) have been recently developed as a novel method to define and estimate causal parameters that depend on the natural value of treatment. LMTPs represent an important advancement in causal inference for longitudinal studies as they allow the non-parametric definition and estimation of the joint effect of multiple categorical, numerical, or continuous exposures measured at several time points. We extend the LMTP methodology to problems in which the outcome is a time-to-event variable subject to right-censoring and competing risks. We present identification results and non-parametric locally efficient estimators that use flexible data-adaptive regression techniques to alleviate model misspecification bias, while retaining important asymptotic properties such as $\sqrt{n}$-consistency. We present an application to the estimation of the effect of the time-to-intubation on acute kidney injury amongst COVID-19 hospitalized patients, where death by other causes is taken to be the competing event.

==> _preamble.tex <==
% for cross-linking documents
\usepackage{nameref,zref-xr} % nameref before zref-xr
\zxrsetup{toltxlabel} % allows use of the \ref command as usual
\usepackage{url}

% math packages
\usepackage{amsmath}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{bm}
\usepackage{bbm}

% journal-specific packages
\makeatletter%
\@ifclassloaded{svjour3}{%
  % for LiDA only
  \usepackage[margin=1in]{geometry}
  \RequirePackage{fix-cm}
  \smartqed  % flush right qed marks, e.g. at end of proof
  %\usepackage[numbers]{natbib}
  %\bibliographystyle{spmpsci}
  \usepackage[round]{natbib}
  %\bibliographystyle{spbasic}
  \bibliographystyle{biometrika}
  \journalname{\textit{Lifetime Data Analysis}}

  \renewenvironment{lemma}{Lemma}{\bfseries}{\itshape}
  \spnewtheorem{assumption}{Condition}{\bfseries}{\itshape}
  \spnewtheorem{assumptioniden}{Assumption}{\bfseries}{\itshape}

   % authorship details
  \newcommand{\authorlist}{
      Iv\'an D\'iaz \and
      Katherine L.~Hoffman \and
      Nima S.~Hejazi
   }
  \authorrunning{I.~D\'iaz et al.} % if too long for running head

  % affiliations
  \institute{
       I.~D\'iaz\at
       Division of Biostatistics\\
       Department of Population Health\\
       New York University Grossman School of Medicine\\
       New York, NY 10016\\
       \email{ivan.diaz@nyu.edu}           %  \\
       %\emph{Present address:} of F. Author  %  if needed
       \and
       K.L.~Hoffman\at
       Department of Biostatistics\\
       University of Washington\\
       Seattle, WA 98195\\
       \email{khof@uw.edu}           %  \\
       \and
       N.S.~Hejazi \at
       Department of Biostatistics\\
       T.H.~Chan School of Public Health\\
       Harvard University\\
       Boston, MA 02115\\
       \email{nhejazi@hsph.harvard.edu}           %  \\
  }
}{%
  %for plain article format only
  \usepackage{arxiv}
  \usepackage{standalone}
  \usepackage[round]{natbib}
  \bibliographystyle{biometrika}
  \usepackage[plain,noend]{algorithm2e}
  \usepackage[colorlinks,citecolor=blue,urlcolor=blue]{hyperref}
  \usepackage{amsthm}

  % math macros incompatible with Springer
  \newtheorem{theorem}{Theorem}
  \newtheorem{remark}{Remark}
  \newtheorem{lemma}{Lemma}
  \newtheorem{proposition}{Proposition}
  \newtheorem{example}{Example}[section]
  \newtheorem{assumption}{}
  \newtheorem{assumptioniden}{}
  \renewcommand\theassumptioniden{{A}\arabic{assumptioniden}}
  \newcommand{\authorlist}{
  Iv\'an D\'iaz \\
  Division of Biostatistics\\
  Department of Population Health\\
  New York University Grossman School of Medicine\\
  \texttt{ivan.diaz@nyu.edu}           
  \And
  Katherine L.~Hoffman \\
  Department of Biostatistics\\
  University of Washington\\
  \texttt{khof@uw.edu}
  \And
  Nima S.~Hejazi \\
  Department of Biostatistics, \\
  T.H.~Chan School of Public Health, \\
  Harvard University \\
  \texttt{nhejazi@hsph.harvard.edu} \\
  }

}
\makeatother

% paper title
%\newcommand{\titlepaper}{Time-to-event analyses with general exposure
%  types and competing risks}
% \newcommand{\titlepaper}{Errata to: ``Causal survival analysis under competing risks using
%   longitudinal modified treatment policies''}

\newcommand{\titlepaper}{Causal survival analysis under competing risks using
  longitudinal modified treatment policies}

% useful packages
\usepackage{float}
\usepackage{graphicx}
% \graphicspath{ {figs/} }
\usepackage{longtable}
\usepackage{color}
\usepackage{multirow}
\usepackage{setspace}
\usepackage{dsfont}
\usepackage[OT1]{fontenc}
\usepackage{refcount}
\usepackage[inline,shortlabels]{enumitem}
\usepackage{booktabs}
\usepackage{accents}
\usepackage{subcaption}

% so so many math macros
\DeclareMathOperator{\expit}{expit}
\DeclareMathOperator{\bern}{Bernoulli}
\DeclareMathOperator{\logit}{logit}
\DeclareMathOperator{\var}{\mathsf{Var}}
\DeclarePairedDelimiter{\norm}{\lVert}{\rVert}
\DeclareMathOperator*{\argmin}{\arg\!\min}
\DeclareMathOperator*{\argmax}{\arg\!\max}
\AtEndDocument{\refstepcounter{theorem}\label{finalthm}}
\AtEndDocument{\refstepcounter{equation}\label{finaleq}}
\renewenvironment{proof}{{\it Proof }}{\qed \\}

\DeclareMathOperator{\opt}{opt}
\DeclareMathOperator{\link}{link}
\newcommand{\hopt}{\hat h_{\opt}}
\newcommand{\supp}{\mathop{\mathrm{supp}}}
\renewcommand\theexample{\arabic{example}}
\newcommand{\pt}{\mbox{$p_0$}}
\newcommand{\pl}{\parallel}

\renewcommand{\P}{\mathsf{P}}
\newcommand{\p}{\mathsf{p}}
\newcommand{\m}{\mathsf{m}}
\newcommand{\q}{\mathsf{q}}
\renewcommand{\r}{\mathsf{z}}
\newcommand{\F}{\mathsf{F}}
\newcommand{\Rem}{\mathsf{J}}
\newcommand{\Remi}{\mathsf{U}}
\renewcommand{\d}{\mathbbm{d}}
\newcommand{\f}{\mathbbm{f}}
\newcommand{\g}{\mathsf{g}}
\renewcommand{\f}{\mathsf{f}}
\renewcommand{\b}{\mathbbm{b}}
\newcommand{\e}{\mathsf{e}}
\newcommand{\uu}{\mathbbm{u}}
\newcommand{\h}{\mathbbm{h}}
\newcommand{\vv}{\mathsf{v}}
\newcommand{\w}{\mathsf{w}}
\newcommand{\G}{\mathsf{G}}
\newcommand{\B}{\mathsf{B}}
\newcommand{\C}{\mathsf{K}}
\renewcommand{\H}{\mathsf{H}}
\newcommand{\W}{\mathsf{W}}

\newcommand{\indep}{\mbox{$\perp\!\!\!\perp$}} \newcommand{\rs}{R}
\newcommand{\ds}{D^\dag} \newcommand{\dd}{\,\mathrm{d}}
\newcommand{\Pn}{\mathsf{P}_n}
\newcommand{\Ps}{\mathsf{P_c}}
\newcommand{\Pnj}{\mathsf{P}_{n,j}}
\newcommand{\Gnj}{\mathsf{G}_{n,j}}
\newcommand{\Gn}{\mathsf{G}_{n}}
\newcommand{\mut}{\mu_0}
\newcommand{\D}{\varphi}
\newcommand{\trie}{\mathsf{D}^{\phi}}
\newcommand{\temp}{\mathsf{D}^{\varphi}}
\newcommand{\cde}{\theta}
\newcommand{\ie}{\phi}
\newcommand{\dcde}{\xi^{\mbox{\scriptsize cde}}}
\newcommand{\die}{\xi^{\mbox{\scriptsize ie}}}
\newcommand{\thetasub}{\hat\theta_{\mbox{\scriptsize sub}}(\delta)}
\newcommand{\thetare}{\hat\theta_{\mbox{\scriptsize re}}(\delta)}
\newcommand{\thetatmle}{\hat\theta_{\mbox{\scriptsize tmle}}}
\newcommand{\thetaos}{\hat\theta_{\mbox{\scriptsize os}}}
\newcommand{\one}{\mathds{1}}
\newcommand{\R}{\mathbb{R}} \renewcommand{\rmdefault}{ptm}
\newcommand{\E}{\mathsf{E}}
\renewcommand{\P}{\mathsf{P}}
\newcommand{\Ec}{\mathbb{E}}
\newcommand{\V}{\mathsf{Var}}
\newcommand{\M}{\mathcal{M}}
\newcommand{\1}{\mathbbm{1}}
\newcommand{\pr}{\mathsf{pr}}
\newcommand{\ubar}[1]{\underaccent{\bar}{#1}}

% editors
\newcommand{\id}[1]{\textcolor{magenta}{*** Iv\'an: #1}}
\newcommand{\nh}[1]{\textcolor{green}{*** Nima: #1}}
\newcommand{\kh}[1]{\textcolor{cyan}{*** Kat: #1}}


% \newcommand{\corr}[1]{\textcolor{magenta}{#1}}
% \newcommand{\corr}[1]{\underline{#1}}
\newcommand{\corr}[1]{#1}
